String stable integral control design for vehicle platoons with disturbances

This paper presents a control design with integral action for vehicle platoons with disturbance that ensures string stability of the closed loop and disturbance rejection. The addition of integral action and a coordinate change allows to develop sufficient smoothness conditions on the closed loop system to ensure that the closed loop system using the proposed controller is string stable in the presence of time-varying disturbances and able able to reject constant disturbances. In addition, bounds for the tracking error of the platoon configuration are also given. Further, a case study is considered together with a suitable controller structure, which satisfies the required smoothness conditions. Simulation results illustrate the performance of the closed loop.

==> figs_v2/5_norms.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8.55}{8.55}\selectfont\strut}%
\psfrag{00000}[cl][cl]{\matlabtextA C1}%
\psfrag{00001}[cl][cl]{\matlabtextA C2}%
\psfrag{0000000000002}[cl][cl]{\matlabtextA Bound (22)}%
\psfrag{0000000000003}[cl][cl]{\matlabtextA Bound (19)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextB Time [s]}%
\psfrag{015}[bc][bc]{\matlabtextB $\sup_i\left|x_i-x_i^*\right|_2$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $10$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $30$}%
\psfrag{008}[ct][ct]{\matlabtextC $40$}%
\psfrag{009}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $10$}%
\psfrag{011}[rc][rc]{\matlabtextC $20$}%
\psfrag{012}[rc][rc]{\matlabtextC $30$}%
\psfrag{013}[rc][rc]{\matlabtextC $40$}%
%
%% </ytick>

==> figs_v2/5delta.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{7.20}{7.20}\selectfont\strut}%
\psfrag{000000}[cl][cl]{\matlabtextA C$_{\textnormal{1}}$}%
\psfrag{000001}[cl][cl]{\matlabtextA C$_{\textnormal{2}}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{034}[tc][tc]{\matlabtextB Time [$s$]}%
\psfrag{035}[bc][bc]{\matlabtextB $e_{i,i-1}$ [m]}%
\psfrag{036}[tc][tc]{\matlabtextB Time [$s$]}%
\psfrag{037}[bc][bc]{\matlabtextB $e_{i,i-1}$ [m]}%
\psfrag{038}[tc][tc]{\matlabtextB Time [$s$]}%
\psfrag{039}[bc][bc]{\matlabtextB $e_{1,0}$ [m]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $5$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $15$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $25$}%
\psfrag{008}[ct][ct]{\matlabtextC $30$}%
\psfrag{013}[ct][ct]{\matlabtextC $0$}%
\psfrag{014}[ct][ct]{\matlabtextC $5$}%
\psfrag{015}[ct][ct]{\matlabtextC $10$}%
\psfrag{016}[ct][ct]{\matlabtextC $15$}%
\psfrag{017}[ct][ct]{\matlabtextC $20$}%
\psfrag{018}[ct][ct]{\matlabtextC $25$}%
\psfrag{019}[ct][ct]{\matlabtextC $30$}%
\psfrag{024}[ct][ct]{\matlabtextC $0$}%
\psfrag{025}[ct][ct]{\matlabtextC $5$}%
\psfrag{026}[ct][ct]{\matlabtextC $10$}%
\psfrag{027}[ct][ct]{\matlabtextC $15$}%
\psfrag{028}[ct][ct]{\matlabtextC $20$}%
\psfrag{029}[ct][ct]{\matlabtextC $25$}%
\psfrag{030}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $-1$}%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $1$}%
\psfrag{012}[rc][rc]{\matlabtextC $2$}%
\psfrag{020}[rc][rc]{\matlabtextC $-1$}%
\psfrag{021}[rc][rc]{\matlabtextC $0$}%
\psfrag{022}[rc][rc]{\matlabtextC $1$}%
\psfrag{023}[rc][rc]{\matlabtextC $2$}%
\psfrag{031}[rc][rc]{\matlabtextC $-2$}%
\psfrag{032}[rc][rc]{\matlabtextC $0$}%
\psfrag{033}[rc][rc]{\matlabtextC $2$}%
%
%% </ytick>

==> figs_v2/5uz.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9.35}{9.35}\selectfont\strut}%
\psfrag{021}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{022}[bc][bc]{\matlabtextA $a_i$ [m/s$^2$]}%
\psfrag{023}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{024}[bc][bc]{\matlabtextA $\dot{q}_i$ [$m/s$]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.50}{8.50}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $25$}%
\psfrag{006}[ct][ct]{\matlabtextB $30$}%
\psfrag{012}[ct][ct]{\matlabtextB $0$}%
\psfrag{013}[ct][ct]{\matlabtextB $5$}%
\psfrag{014}[ct][ct]{\matlabtextB $10$}%
\psfrag{015}[ct][ct]{\matlabtextB $15$}%
\psfrag{016}[ct][ct]{\matlabtextB $20$}%
\psfrag{017}[ct][ct]{\matlabtextB $25$}%
\psfrag{018}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $-3$}%
\psfrag{008}[rc][rc]{\matlabtextB $-2$}%
\psfrag{009}[rc][rc]{\matlabtextB $-1$}%
\psfrag{010}[rc][rc]{\matlabtextB $0$}%
\psfrag{011}[rc][rc]{\matlabtextB $1$}%
\psfrag{019}[rc][rc]{\matlabtextB $20$}%
\psfrag{020}[rc][rc]{\matlabtextB $22$}%
%
%% </ytick>

==> figs_v2/5z3.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{032}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{033}[bc][bc]{\matlabtextA $\zeta_i$}%
\psfrag{034}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{035}[bc][bc]{\matlabtextA $a_i$ [m/s$^2$]}%
\psfrag{036}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{037}[bc][bc]{\matlabtextA $\dot{q}_i$ [$m/s$]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $25$}%
\psfrag{006}[ct][ct]{\matlabtextB $30$}%
\psfrag{011}[ct][ct]{\matlabtextB $0$}%
\psfrag{012}[ct][ct]{\matlabtextB $5$}%
\psfrag{013}[ct][ct]{\matlabtextB $10$}%
\psfrag{014}[ct][ct]{\matlabtextB $15$}%
\psfrag{015}[ct][ct]{\matlabtextB $20$}%
\psfrag{016}[ct][ct]{\matlabtextB $25$}%
\psfrag{017}[ct][ct]{\matlabtextB $30$}%
\psfrag{023}[ct][ct]{\matlabtextB $0$}%
\psfrag{024}[ct][ct]{\matlabtextB $5$}%
\psfrag{025}[ct][ct]{\matlabtextB $10$}%
\psfrag{026}[ct][ct]{\matlabtextB $15$}%
\psfrag{027}[ct][ct]{\matlabtextB $20$}%
\psfrag{028}[ct][ct]{\matlabtextB $25$}%
\psfrag{029}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $-6$}%
\psfrag{008}[rc][rc]{\matlabtextB $-4$}%
\psfrag{009}[rc][rc]{\matlabtextB $-2$}%
\psfrag{010}[rc][rc]{\matlabtextB $0$}%
\psfrag{018}[rc][rc]{\matlabtextB $-3$}%
\psfrag{019}[rc][rc]{\matlabtextB $-2$}%
\psfrag{020}[rc][rc]{\matlabtextB $-1$}%
\psfrag{021}[rc][rc]{\matlabtextB $0$}%
\psfrag{022}[rc][rc]{\matlabtextB $1$}%
\psfrag{030}[rc][rc]{\matlabtextB $20$}%
\psfrag{031}[rc][rc]{\matlabtextB $22$}%
%
%% </ytick>

==> figures/100_norms.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8.55}{8.55}\selectfont\strut}%
\psfrag{00000000000000}[cl][cl]{\matlabtextA State Error}%
\psfrag{000000000001}[cl][cl]{\matlabtextA Our Bound}%
\psfrag{000000000000000002}[cl][cl]{\matlabtextA Monteil's Bound}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{011}[tc][tc]{\matlabtextB Time [s]}%
\psfrag{012}[bc][bc]{\matlabtextB $\sup_i\left|z-z^*\right|_2$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $20$}%
\psfrag{006}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $100$}%
\psfrag{009}[rc][rc]{\matlabtextC $200$}%
\psfrag{010}[rc][rc]{\matlabtextC $300$}%
%
%% </ytick>

==> figures/100delta.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{021}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{022}[bc][bc]{\matlabtextA $\delta_{i,i-1}$ [m]}%
\psfrag{023}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{024}[bc][bc]{\matlabtextA $\delta_{1,0}$ [m]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $25$}%
\psfrag{006}[ct][ct]{\matlabtextB $30$}%
\psfrag{011}[ct][ct]{\matlabtextB $0$}%
\psfrag{012}[ct][ct]{\matlabtextB $5$}%
\psfrag{013}[ct][ct]{\matlabtextB $10$}%
\psfrag{014}[ct][ct]{\matlabtextB $15$}%
\psfrag{015}[ct][ct]{\matlabtextB $20$}%
\psfrag{016}[ct][ct]{\matlabtextB $25$}%
\psfrag{017}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $-20$}%
\psfrag{008}[rc][rc]{\matlabtextB $-10$}%
\psfrag{009}[rc][rc]{\matlabtextB $0$}%
\psfrag{010}[rc][rc]{\matlabtextB $10$}%
\psfrag{018}[rc][rc]{\matlabtextB $-1$}%
\psfrag{019}[rc][rc]{\matlabtextB $0$}%
\psfrag{020}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> figures/100speed.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{006}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{007}[bc][bc]{\matlabtextA $\dot{q}_i$ [$m/s$]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $0$}%
\psfrag{005}[rc][rc]{\matlabtextB $20$}%
%
%% </ytick>

==> figures/100uz.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{015}[bc][bc]{\matlabtextA $u_{\zeta,i}$ [m/s$^2$]}%
\psfrag{016}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{017}[bc][bc]{\matlabtextA $u_{a,i}$ [m/s$^2$]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{007}[ct][ct]{\matlabtextB $0$}%
\psfrag{008}[ct][ct]{\matlabtextB $10$}%
\psfrag{009}[ct][ct]{\matlabtextB $20$}%
\psfrag{010}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $-10$}%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $10$}%
\psfrag{011}[rc][rc]{\matlabtextB $-5$}%
\psfrag{012}[rc][rc]{\matlabtextB $0$}%
\psfrag{013}[rc][rc]{\matlabtextB $5$}%
%
%% </ytick>

==> figures/100z3.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{019}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{020}[bc][bc]{\matlabtextA $\zeta_i$}%
\psfrag{021}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{022}[bc][bc]{\matlabtextA $\dot{q}_i$ [$m/s$]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $25$}%
\psfrag{006}[ct][ct]{\matlabtextB $30$}%
\psfrag{009}[ct][ct]{\matlabtextB $0$}%
\psfrag{010}[ct][ct]{\matlabtextB $5$}%
\psfrag{011}[ct][ct]{\matlabtextB $10$}%
\psfrag{012}[ct][ct]{\matlabtextB $15$}%
\psfrag{013}[ct][ct]{\matlabtextB $20$}%
\psfrag{014}[ct][ct]{\matlabtextB $25$}%
\psfrag{015}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $20$}%
\psfrag{016}[rc][rc]{\matlabtextB $-20$}%
\psfrag{017}[rc][rc]{\matlabtextB $-10$}%
\psfrag{018}[rc][rc]{\matlabtextB $0$}%
%
%% </ytick>

==> figures/200_norms.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8.55}{8.55}\selectfont\strut}%
\psfrag{000000000}[cl][cl]{\matlabtextA C$_{\textnormal{1}}$ SE}%
\psfrag{000000001}[cl][cl]{\matlabtextA C$_{\textnormal{2}}$ SE}%
\psfrag{00000002}[cl][cl]{\matlabtextA C$_{\textnormal{1}}$ B}%
\psfrag{00000003}[cl][cl]{\matlabtextA C$_{\textnormal{2}}$ B}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextB Time [s]}%
\psfrag{015}[bc][bc]{\matlabtextB $\sup_i\left|x_i-x_i^*\right|_2$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $10$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $30$}%
\psfrag{008}[ct][ct]{\matlabtextC $40$}%
\psfrag{009}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $50$}%
\psfrag{012}[rc][rc]{\matlabtextC $100$}%
\psfrag{013}[rc][rc]{\matlabtextC $150$}%
%
%% </ytick>

==> figures/25_norms.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8.55}{8.55}\selectfont\strut}%
\psfrag{000000}[cl][cl]{\matlabtextA C$_{\textnormal{1}}$}%
\psfrag{000001}[cl][cl]{\matlabtextA C$_{\textnormal{2}}$}%
\psfrag{0000000000002}[cl][cl]{\matlabtextA Bound (21)}%
\psfrag{0000000000003}[cl][cl]{\matlabtextA Bound (18)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{016}[tc][tc]{\matlabtextB Time [s]}%
\psfrag{017}[bc][bc]{\matlabtextB $\sup_i\left|x_i-x_i^*\right|_2$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $10$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $30$}%
\psfrag{008}[ct][ct]{\matlabtextC $40$}%
\psfrag{009}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $20$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $60$}%
\psfrag{013}[rc][rc]{\matlabtextC $80$}%
\psfrag{014}[rc][rc]{\matlabtextC $100$}%
\psfrag{015}[rc][rc]{\matlabtextC $120$}%
%
%% </ytick>

==> figures/25delta.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{7.20}{7.20}\selectfont\strut}%
\psfrag{000000}[cl][cl]{\matlabtextA C$_{\textnormal{1}}$}%
\psfrag{000001}[cl][cl]{\matlabtextA C$_{\textnormal{2}}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{029}[tc][tc]{\matlabtextB Time [$s$]}%
\psfrag{030}[bc][bc]{\matlabtextB $e_{i,i-1}$ [m]}%
\psfrag{031}[tc][tc]{\matlabtextB Time [$s$]}%
\psfrag{032}[bc][bc]{\matlabtextB $e_{i,i-1}$ [m]}%
\psfrag{033}[tc][tc]{\matlabtextB Time [$s$]}%
\psfrag{034}[bc][bc]{\matlabtextB $e_{1,0}$ [m]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $10$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $40$}%
\psfrag{007}[ct][ct]{\matlabtextC $50$}%
\psfrag{011}[ct][ct]{\matlabtextC $0$}%
\psfrag{012}[ct][ct]{\matlabtextC $10$}%
\psfrag{013}[ct][ct]{\matlabtextC $20$}%
\psfrag{014}[ct][ct]{\matlabtextC $30$}%
\psfrag{015}[ct][ct]{\matlabtextC $40$}%
\psfrag{016}[ct][ct]{\matlabtextC $50$}%
\psfrag{020}[ct][ct]{\matlabtextC $0$}%
\psfrag{021}[ct][ct]{\matlabtextC $10$}%
\psfrag{022}[ct][ct]{\matlabtextC $20$}%
\psfrag{023}[ct][ct]{\matlabtextC $30$}%
\psfrag{024}[ct][ct]{\matlabtextC $40$}%
\psfrag{025}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $-20$}%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $-2$}%
\psfrag{018}[rc][rc]{\matlabtextC $0$}%
\psfrag{019}[rc][rc]{\matlabtextC $2$}%
\psfrag{026}[rc][rc]{\matlabtextC $-1$}%
\psfrag{027}[rc][rc]{\matlabtextC $0$}%
\psfrag{028}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> figures/25uz.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{010}[bc][bc]{\matlabtextA $u_{a,i}$ [m/s$^2$]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $-10$}%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $10$}%
%
%% </ytick>

==> figures/25z3.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{017}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{018}[bc][bc]{\matlabtextA $\zeta_i$}%
\psfrag{019}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{020}[bc][bc]{\matlabtextA $\dot{q}_i$ [$m/s$]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
\psfrag{008}[ct][ct]{\matlabtextB $0$}%
\psfrag{009}[ct][ct]{\matlabtextB $10$}%
\psfrag{010}[ct][ct]{\matlabtextB $20$}%
\psfrag{011}[ct][ct]{\matlabtextB $30$}%
\psfrag{012}[ct][ct]{\matlabtextB $40$}%
\psfrag{013}[ct][ct]{\matlabtextB $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $0$}%
\psfrag{007}[rc][rc]{\matlabtextB $20$}%
\psfrag{014}[rc][rc]{\matlabtextB $-20$}%
\psfrag{015}[rc][rc]{\matlabtextB $-10$}%
\psfrag{016}[rc][rc]{\matlabtextB $0$}%
%
%% </ytick>

==> figures/normsN.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{007}[tc][tc]{\matlabtextA N}%
\psfrag{008}[bc][bc]{\matlabtextA $\sup_i\left|z_i-z_i^*\right|_\infty$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $25$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{001}[rc][rc]{\matlabtextB $0$}%
\psfrag{002}[rc][rc]{\matlabtextB $5$}%
\psfrag{003}[rc][rc]{\matlabtextB $10$}%
\psfrag{004}[rc][rc]{\matlabtextB $15$}%
\psfrag{005}[rc][rc]{\matlabtextB $20$}%
\psfrag{006}[rc][rc]{\matlabtextB $25$}%
%
%% </ytick>
